Imagine That! Leveraging Emergent Affordances for 3D Tool Synthesis

In this paper we explore the richness of information captured by the latent space of a vision-based generative model. The model combines unsupervised generative learning with a task-based performance predictor to learn and to exploit task-relevant object affordances given visual observations from a reaching task, involving a scenario and a stick-like tool. While the learned embedding of the generative model captures factors of variation in 3D tool geometry (e.g. length, width, and shape), the performance predictor identifies sub-manifolds of the embedding that correlate with task success. Within a variety of scenarios, we demonstrate that traversing the latent space via backpropagation from the performance predictor allows us to imagine tools appropriate for the task at hand. Our results indicate that affordances-like the utility for reaching-are encoded along smooth trajectories in latent space. Accessing these emergent affordances by considering only high-level performance criteria (such as task success) enables an agent to manipulate tool geometries in a targeted and deliberate way.

==> archive/notes.tex <==
%abstract

\begin{abstract}
%NEW VERSION (emphasises affordances over tools, following ICML workshop paper)
In this paper we explore the richness of information captured by the latent space of a novel, vision-based generative model. %, how this information is shaped by a task, and how the latent space can be searched in a directed way to imagine novel solutions. 
%
The model combines unsupervised generative learning with a task-based performance predictor to learn and to exploit task-relevant object \emph{affordances} given visual observations from a reaching task, involving a scenario and a stick-like tool. % and stick-like tool. 
%
While the learned embedding of the generative model captures factors of variation in 3D tool geometry (e.g.~length, width, and shape), the performance predictor identifies sub-manifolds of the embedding that correlate with task success. % in a weakly supervised manner. 
%
%Using a 3D simulation environment 
Within a variety of scenarios, we demonstrate that traversing the latent space via backpropagation from the performance predictor allows us to \emph{imagine} tools appropriate for the task at hand. 
%
Our results indicate that affordances -- like the utility for reaching -- are encoded along smooth trajectories in latent space. 
%
Accessing these emergent affordances by considering only \emph{high-level} performance criteria (such as task success) enables an agent to manipulate tool geometries in a targeted and deliberate way. %stronger claim if replace `tool geometries'? e.g. latent representations and renderings?
% %OLD VERSION (BMVC)
% In this paper we explore the richness of information captured by the latent space of a vision-based generative model -- and how to exploit it. The context of our work is an artificial agent's ability to perform task-focused \emph{tool~synthesis} for 3D reaching tasks based purely on 2D visual inputs. In particular, given visual observations of a reaching task and a proposed tool, our approach employs activation maximisation of a task-based performance predictor to directly optimise the 3D  geometry of the tool by traversing a learnt latent space. While the embedding learned by the generative model captures the factors of variation in 3D tool geometry, e.g.~length, width and configuration, the performance predictor identifies sub-manifolds correlated with task success in a weakly supervised manner. Using a 3D simulation environment, we demonstrate that traversing the latent space in this task-driven way results in tool geometries appropriate for the task at hand. Our results therefore suggest that affordances -- like the utility for reaching -- are encoded along smooth trajectories in the learned latent space. Accessing these emergent affordances via gradient descent considering only \emph{high-level} performance criteria (such as task success) enables the agent to manipulate tool geometries in a targeted and deliberate way. https://ori.ox.ac.uk/tool\_imagination/
\end{abstract}

==> secdataset.tex <==
To investigate tool imagination, we designed a set of simulated reaching tasks with clear and controllable factors of influence.
Each task image is comprised of a green target button, three red lines delineating the workspace area, and, optionally, a set of blue obstacles. We also vary the goal location and the sizes and positions of the obstacles. For each task image, we provide a second image depicting a tool, i.e. a straight stick or a L-shaped hook, with varying dimensions, shapes, and textures. Given a pair of images (i.e. the task image and  the tool image), the goal is to predict whether the tool for a given task scene can reach the target (the green dot) whilst avoiding obstacles (blue areas) and remaining on the exterior of the workspace (i.e.~behind the red line).
%
Depending on the task image, the applicability of a tool is determined by different subsets of its attributes. For example, if the target button is unobstructed, then any tool of sufficient length will satisfy the constraints (regardless of its width or shape).
However, when the target is hidden behind a corner, or only accessible through a narrow gap, an appropriate tool also needs to feature a long-enough hook, or a thin-enough handle, respectively.
%
As depicted in Figure \ref{fig:dataset}, we have designed five scenario types to study these factors of influence in isolation and in combination. The task setting and the tool are first rendered in a top-down view for the geometric applicability check. Then the tool is rendered in 12 different views for the 3D reconstruction.
%
The geometric applicability check, described in Supplementary materials, verifies whether or not any of the tools can reach the target, while satisfying the task constraints.
%Appendix~\ref{sec:dataset_sup}

More formally, our dataset can be written as a set of $N$ instances: $\{ (I_G^{n}, I_T^{n,i}, I_T^{n,j}, I_S^{n,i}, I_S^{n,j},$
$ \rho^{n}) \}_{n=1}^{N}$, where each example features a task image $I_G$, tool images $I_T$ in two randomly selected views $i$ and $j$, and their corresponding silhouette $I_S$, as well as a binary label $\rho$ indicating the feasibility of reaching the target with the given tool.
%
In all our experiments, we restrict the training input to the sparse high-level instances. For additional details on the dataset, see Supplementary materials.%~\ref{sec:dataset_sup}.

% \begin{figure}[t!]
% \centering
% \includegraphics[width=\textwidth]{images/fig_dataset.png}
% \caption{
% % OLD VERSION
% % Examples of tasks in our dataset. 
% % %
% % The first block of \textit{in-sample scenario types} (\texttt{A} -- \texttt{D}) were used for training. 
% % %
% % The second block of \textit{interpolation scenario types} (\texttt{E} -- \texttt{G}) were used for evaluation and could be solved with (unseen) sticks and hooks, which are tool types seen during training. 
% % %
% % The third block of \textit{extrapolation scenario type} (\texttt{H}) were also used for evaluation but required a novel claw-shaped tool type. 
% % %
% % By design, these scenarios impose constraints on successful tools, affecting the properties of length, width, and configuration. 
% % %
% % For example, \texttt{B} requires a hook instead of a stick.
% % %
% % Green ticks appear next to successful tools (top row) while red crosses denote failures (bottom row). 
% % %
% % The same tasks are repeated in top and bottom rows in each column. 
% %SASHA
% (Left) Task examples from our dataset. Top and bottom rows correspond to unsuccessful and successful tool examples respectively. Columns A-E represent 5 different task scenario types each imposing different tool constraints including width, length, orientation and shape. (Right) Model inputs \{task observation, tool observation\}.
% } \label{fig:dataset}
% \end{figure}



